Incorporating Vision Bias into Click Models for Image-oriented Search Engine

Most typical click models assume that the probability of a document to be examined by users only depends on position, such as PBM and UBM. It works well in various kinds of search engines. However, in a search engine where massive candidate documents display images as responses to the query, the examination probability should not only depend on position. The visual appearance of an image-oriented document also plays an important role in its opportunity to be examined. In this paper, we assume that vision bias exists in an image-oriented search engine as another crucial factor affecting the examination probability aside from position. Specifically, we apply this assumption to classical click models and propose an extended model, to better capture the examination probabilities of documents. We use regression-based EM algorithm to predict the vision bias given the visual features extracted from candidate documents. Empirically, we evaluate our model on a dataset developed from a real-world online image-oriented search engine, and demonstrate that our proposed model can achieve significant improvements over its baseline model in data fitness and sparsity handling.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> ori_perplexity.tex <==
Besides, because \cite{UBM} suggests that predicting skips is usually an easier task compared with predicting clicks, we also compute perplexity for clicked documents. 
We also report the perplexity improvement over extended models for each rank in Figure \ref{perp_rank}. We observe that regression-based EM algorithm improves the performance at higher ranks. In our dataset, not all search sessions have the same number of documents. Higher rank means less training data. Thus, with less sparse training data, regression-based EM algorithm performs better than standard EM algorithm.

\begin{figure} 
  \centering
  \includegraphics[width=0.5\textwidth]{perp.pdf}
  \caption{Improvements of perplexity at each rank.}
  \Description{Improvements of perplexity at each rank over UBM.}
  \label{perp_rank}
\end{figure}
\begin{figure} 
  \centering
  \includegraphics[width=0.5\textwidth]{clicked_perp.pdf}
  \caption{Perplexity at clicked documents.}
  \Description{Perplexity at clicked documents.}
  \label{perp_clicked}
\end{figure}

\par
Next we analyze the performance at clicked documents. In our dataset, for every six documents, there is one document getting clicked on average. Thus, the training data for clicked documents is less than that for unclicked documents. In Figure \ref{perp_clicked}, we compare both total perplexity and perplexity at clicked documents. Extended UBM models improve not only on total perplexity, but also on perplexity for clicked documents. Table \ref{improv_clicked} shows the improvements of perplexities at clicked documents for each model. While all models achieve significant improvements over UBM, regression-based EM algorithm performs better than standard EM algorithm. When we filter more sparse queries for GBDT in regression-based EM algorithm, the perplexity improves. It proves the ability of our model to handle data sparsity problem. 
\par
In Table \ref{perp_fre}, we compare the perplexity on different query frequencies, where \textit{vUBM-R} has better performance than \textit{vUBM-S}. As is shown in Table \ref{imp_fre}, for any $vUBM-R$ model using regression-based EM algorithm, the perplexity on queries appearing for less than 10 times in the training dataset has higher improvement over \textit{vUBM-S}. Regression-based EM algorithm handles sparse queries better than standard EM algorithm.
\begin{table}
  \caption{Improvements on perplexity at clicked documents over UBM.}
  \label{improv_clicked}
  \begin{tabular}{p{1.5cm}p{3cm}p{3cm}}
    \toprule
    &Perplexity&Improvement\\
    \midrule
    UBM&1.1746&-\\
    vUBM-S&1.1706&+2.29\%\\
    vUBM-R\_1&1.1660&+4.93\%\\
    vUBM-R\_2&1.1596&+8.59\%\\
    vUBM-R\_3&1.1596&+8.59\%\\
    vUBM-R\_5&\textbf{1.1587}&+\textbf{9.11}\%\\
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Perplexity for different query frequencies.}
  \label{perp_fre}
  \begin{tabular}{p{1.5cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
    \toprule
    &1-10&10-100&100-1000&1000-10000\\
    \midrule
    vUBM-S&1.2911&1.2510&1.2752&1.2761\\
    vUBM-R\_1&1.2884&1.2514&1.2738&1.2733\\
    vUBM-R\_2&1.2873&1.2507&1.2732&1.2727\\
    vUBM-R\_3&1.2873&1.2505&1.2729&1.2726\\
    vUBM-R\_5&\textbf{1.2871}&\textbf{1.2504}&\textbf{1.2725}&\textbf{1.2724}\\
  \bottomrule
\end{tabular}
\end{table}
\begin{table}
  \caption{Improvement of perplexity of \textit{vUBM-R} for different query frequencies over \textit{vUBM-S}.}
  \label{imp_fre}
  \begin{tabular}{p{1.5cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
    \toprule
    &1-10&10-100&100-1000&1000-10000\\
    \midrule
    vUBM-R\_1&+0.93\%&-1.59\%&+0.51\%&\textbf{+1.01\%}\\
    vUBM-R\_2&\textbf{+1.31\%}&+0.12\%&+0.73\%&+1.23\%\\
    vUBM-R\_3&\textbf{+1.31\%}&+0.20\%&+0.84\%&+1.27\%\\
    vUBM-R\_5&\textbf{+1.37\%}&+0.24\%&+0.98\%&+1.34\%\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Baseline Models}
In this paper, two baseline models, PBM and UBM are used for comparison. PBM assumes that opportunity to be examined for a document depends on its position, and a document is clicked if and only if the user examines the document and recognizes that the document is relevant. The relevance of a document only depends on the query and the document itself. 
\par
Formally, PBM has the following assumptions:
 \begin{equation}
C_{r} = 1 \Leftrightarrow{} E_{r} = 1, R_{r} = 1
\end{equation}
 \begin{equation}
P\left(R_{r} = 1\right) = \alpha_{_{qd}}
\end{equation}
 \begin{equation}
P\left(E_{r} = 1\right) = \gamma_{_{r}}\label{exmination_0}
\end{equation}
The click probability for a given document $d$ at rank $r$ can be calculated by the following equation.
\begin{equation}
P \left( C_{r} = 1 \right) = \alpha_{_{qd}}\gamma_{_{r}} 
\end{equation}
UBM is developed based on PBM. Not like the original examination hypothesis used in PBM, UBM supposes that the opportunity to be examined for a document depends on both its position and the position of the previously clicked document. According to the assumptions of UBM, a document is clicked if and only if the user examines the document and recognizes that the document is relevant. In a search session with $N$ documents, the examination probability of a document at rank $r$ ($1 \leq r \leq N$) is decided by $r$ and $r'$, where the previous click happens ($r'$ = 0 if no previous documents are clicked). For a query $q$ and a displayed document $d$, the relevance only depends on $q$ and $d$. 
\par
 Formally, UBM has the following assumptions:
 \par
 \begin{equation}
C_{r} = 1 \Leftrightarrow{} E_{r} = 1, R_{r} = 1
\end{equation}
 \begin{equation}
P\left(R_{r} = 1\right) = \alpha_{_{qd}}
\end{equation}
 \begin{equation}
P\left(E_{r} = 1 \mid C_{1} = c_{1}, ..., C_{r-1} = c_{r-1}\right) = \gamma_{_{rr'}}\label{exmination}
\end{equation}
 \begin{displaymath}
 r' = max \{k \in \{ 0, ..., r-1 \}:  c_{k} = 1\}
\end{displaymath}
Following the assumptions above, the click probability for a given document $d$ at rank $r$ can be calculated by the following equation.
\begin{equation}
P \left( C_{r} = 1 \right) = \alpha_{_{qd}}\gamma_{_{rr'}} 
\end{equation}


